Breaking the Script Barrier in Multilingual Pre-Trained Language Models with Transliteration-Based Post-Training Alignment

Multilingual pre-trained models (mPLMs) have shown impressive performance on cross-lingual transfer tasks. However, the transfer performance is often hindered when a low-resource target language is written in a different script than the high-resource source language, even though the two languages may be related or share parts of their vocabularies. Inspired by recent work that uses transliteration to address this problem, our paper proposes a transliteration-based post-pretraining alignment (PPA) method aiming to improve the cross-lingual alignment between languages using diverse scripts. We select two areal language groups, $\textbf{Mediterranean-Amharic-Farsi}$ and $\textbf{South+East Asian Languages}$, wherein the languages are mutually influenced but use different scripts. We apply our method to these language groups and conduct extensive experiments on a spectrum of downstream tasks. The results show that after PPA, models consistently outperform the original model (up to 50% for some tasks) in English-centric transfer. In addition, when we use languages other than English as sources in transfer, our method obtains even larger improvements. We will make our code and models publicly available at \url{https://github.com/cisnlp/Transliteration-PPA}.

==> old_intro.tex <==
%Self-supervised pre-trained masked language models (MLMs) like BERT~\citep{devlin-etal-2019-bert} and RoBERTa~\citep{liu2019roberta}
%have found incredible success in transfer learning across a wide range of NLP tasks.
Pre-trained multilingual masked language models (MMLMs) such as mBERT~\citep{devlin-etal-2019-bert} and XLM-R~\citep{conneau-etal-2020-unsupervised}
have shown remarkable performance on cross-lingual transfer tasks by learning cross-lingual representations from monolingual corpora~\citep{pires-etal-2019-multilingual, artetxe-etal-2020-cross}.
A notable extension of these models is Glot500~\citep{imanigooghari-etal-2023-glot500}, which adapted
XLM-R to support more than 500 languages, thus significantly improving performance on low-resource languages.

%\citet{cao2019multilingual} showed that the downstream performance of
%multilingual models is correlated with the degree of alignment between word embeddings across languages. \citet{deshpande-etal-2022-bert}
%also confirmed this observation and further showed that absence of subword overlap hinders cross-lingual transfer when the source and target
%languages differ in their word order.

%Another factor that hurts the downstream performance of multilingual models is the script diversity of represented languages.
%This has been observed even in the case of related languages, if the source and target languages are written in different scripts
%~\citep{muller-etal-2021-unseen, anastasopoulos-neubig-2019-pushing}. We can also view the script barrier problem from the lens of
%representation alignment. \citet{wen-yi-mimno-2023-hyperpolyglot} showed that XLM-R embeddings of tokens from different scripts
%can be almost perfectly linearly separated. This indicates that multilingual encoder models struggle to learn a common representation space
%across different scripts, thus requiring additional post-training alignment.

Despite their impressive performance, these models still exhibit limitations in cross-lingual transfer, especially for low-resource languages.
These weaknesses have been studied from different perspectives. \citet{deshpande-etal-2022-bert} showed that the downstream performance of
multilingual models is correlated with the degree of alignment between word embeddings across languages. Another factor that hinders the
knowledge transfer is the script diversity of represented languages, which has been observed even in the case of
related languages~\citep{muller-etal-2021-unseen, anastasopoulos-neubig-2019-pushing}. The script barrier problem can also be viewed from
the lens of representation alignment. \citet{wen-yi-mimno-2023-hyperpolyglot} showed that XLM-R embeddings of tokens from different scripts
can be almost perfectly linearly separated, indicating that multilingual encoder models struggle to learn a common representation space
across different scripts, thus requiring additional post-training alignment.

%As the number of languages and scripts in the multilingual models increases, the importance of better aligning representations
%becomes more pronounced. Low-resource languages written in underrepresented scripts are especially affected, as the models have limited
%capacity to learn useful representations for these languages. The downstream performance on these languages can be significantly improved
%by aligning their representations with related high-resource languages. Recent works have proposed additional alignment supervision
%signals that can be used to improve the cross-lingual transfer performance of multilingual models
%\citep{pan-etal-2021-multilingual, cao2019multilingual, hu-etal-2021-explicit}.
%This line of research however relies on parallel data or bilingual dictionaries in order to align word embeddings across languages.

%An alternative approach for improving cross-lingual transfer in multilingual models is to apply transliteration, a process of converting
%language text from one script to another. By pre-training or fine-tuning models with data transliterated into a common script,
%several works have shown improvements in downstream task performance
%\citep{muller-etal-2021-unseen, murikinati-etal-2020-transliteration, purkayastha-etal-2023-romanization, moosa-etal-2023-transliteration}.
%However, these works force a common script limitation on the model, which can be restrictive for specific tasks as the process of
%transliteration can be lossy and non-invertible.
%% Need advice on how to better present the next paragraphs
%Recently, \citet{liu2024translico} proposed a sequence-level contrastive learning method on original and transliterated data
%that can be used to improve cross-lingual transfer performance across different languages and scripts. However, this method is limited to
%only sentence-level alignment by means of in-batch contrastive learning. This objective can be very easy for the model to learn, in the
%absence of hard negative examples, and may not be sufficient for improving the alignment at the word/token level.

As the number of languages and scripts in the multilingual models increases, the importance of better aligning representations
becomes more pronounced. Recent works have proposed additional alignment supervision signals that can be used to improve the cross-lingual transfer performance of
multilingual models~\citep{pan-etal-2021-multilingual, cao2019multilingual, hu-etal-2021-explicit}. However,
this line of research relies on parallel data or bilingual dictionaries in order to align word embeddings across languages.
An alternative approach that does not rely on parallel data is to apply transliteration, a process of converting language text from one script to another.
Several works have shown improvements in cross-lingual transfer by pre-training or fine-tuning models with data transliterated into a common script
~\citep{muller-etal-2021-unseen, murikinati-etal-2020-transliteration, purkayastha-etal-2023-romanization, moosa-etal-2023-transliteration}.
However, these works impose a common script limitation on the model, which can be restrictive for specific tasks as the process of transliteration
can be lossy and non-invertible. Recently, \citet{liu2024translico} proposed a sequence-level contrastive learning method based on original and
transliterated data.
%TODO: how to attack Translico in the intro?
% the sequence-level task does not directly contribute to the alignment in the token space.

% change the order
In this work, we investigate the impact of transliteration-based alignment on cross-lingual transfer by focusing on two groups of languages.
The languages in each group are selected so that they differ in scripts and share some similarities. Some of the languages are closely related
by belonging to the same language family (e.g, Arabic, Hebrew, and Maltese). Others share some lexical overlap due to historical contact
and geographical proximity (e.g, Chinese and Korean, or Turkish and Arabic). As these languages are written in different scripts, transliteration
can help to better exploit the shared linguistic properties and as a result improve the cross-lingual transfer performance of multilingual models.
The two groups of languages, which we name \textbf{Mediterranean-Arabic Languages} and \textbf{South-East Asian Languages}, are described in
more detail in Section~\ref{subsec:languages-and-data}.

Our proposed transliteration-based alignment method aims to bridge the script barrier in multilingual models by aligning the representations
of languages written in different scripts. We combine masked language modeling, sentence-level alignment, and token-level alignment objectives
on original and transliterated data. The architecture of the proposed method is shown in Figure~\ref{fig:architecture}.
This method does not rely on parallel data, and we use Uroman~\citep{hermjakob-etal-2018-box} to efficiently transliterate monolingual data
into a common Latin script. We fine-tune the Glot500 model on the selected languages and evaluate the cross-lingual transfer performance
on several downstream tasks. The evaluation is done with English as the source language, as well as with three other source languages of different scripts
for each group of languages. We show that our method can improve the downstream task performance across different languages and scripts,
thus demonstrating the effectiveness of transliteration-based alignment for multilingual models. Moreover, we observe the importance of choosing
the right source language for transfer, as the performance can vary significantly depending on the script and degree of similarity between the source and target languages.
Our contributions can be summarized as follows:

\begin{figure*}[htb!]
\centering
\includegraphics[width=0.8\textwidth]{plots/architecture}
\caption{Architecture of the proposed transliteration-based alignment method.}
\label{fig:architecture}
\end{figure*}

1. We propose a post-training transliteration-based alignment method aiming to bridge the script barrier problem in multilingual models.

2. We investigate the impact of transliteration-based alignment on two groups of similar languages with different scripts and show improvements in cross-lingual transfer performance.

3. We conduct a systematic evaluation on how different source languages influence the transfer of transliteration-aligned models.

\section{Related Work}\label{sec:related-work}
Many recent works have proposed pre-training or fine-tuning alignment methods to improve cross-lingual transfer in multilingual models.
\citet{chaudhary2020dict} improved alignment during pre-training by using bilingual dictionaries to replace words in original sentences
with their translations in other languages. \citet{tang2022align, cao2019multilingual} proposed explicit embedding alignment objectives
between words acquired from bilingual dictionaries. \citet{hu-etal-2021-explicit} proposed a pre-training method with explicit alignment signals
from parallel data that encourages symmetry at both word and sentence levels. Similarly, \citet{wei2020learning} proposed a hierarchical
contrastive learning pre-training method, which aligns representations at the word and sentence levels by using parallel data.
\citet{pan-etal-2021-multilingual} combined contrastive learning with translation language modeling (TLM)~\citep{conneau2019cross} as a post-training
alignment method also using parallel data. While these methods have shown improvements, they have the limitation of requiring parallel data or bilingual dictionaries
which may be hard to acquire for low-resource languages.

Different works have proposed transliteration-based methods in order to address the script barrier problem in multilingual models.
\citet{khemchandani-etal-2021-exploiting} exploited language relatedness between Indian languages, and utilized transliteration to a common script
in order to adapt multilingual models to low-resource languages. \citet{murikinati-etal-2020-transliteration} used transliteration to a common script
to improve cross-lingual morphological inflection. \citet{muller-etal-2021-unseen} analysed the behavior of multilingual models on unseen languages, and found that
languages written in different scripts do not benefit from transfer learning. They proposed transliteration to the high-resource source language script as a solution to address
the script barrier. \citet{purkayastha-etal-2023-romanization} showed that fine-tuning of multilingual models on data transliterated into Latin script improves cross-lingual transfer
for low-resource languages. Similarly, \citet{moosa-etal-2023-transliteration} pre-trained models from scratch on data transliterated into a common script for the Indic languages and
showed improvements in cross-lingual transfer and alignment. \citet{liu2024translico} proposed a sequence-level contrastive learning objective
on original and transliterated data to encourage alignment across different scripts without the restriction of adapting models to a common script.
%TODO: some words about how our method is different
